Automatic Integration for Spatiotemporal Neural Point Processes

Learning continuous-time point processes is essential to many discrete event forecasting tasks. However, integration poses a major challenge, particularly for spatiotemporal point processes (STPPs), as it involves calculating the likelihood through triple integrals over space and time. Existing methods for integrating STPP either assume a parametric form of the intensity function, which lacks flexibility; or approximating the intensity with Monte Carlo sampling, which introduces numerical errors. Recent work by Omi et al. [2019] proposes a dual network approach for efficient integration of flexible intensity function. However, their method only focuses on the 1D temporal point process. In this paper, we introduce a novel paradigm: AutoSTPP (Automatic Integration for Spatiotemporal Neural Point Processes) that extends the dual network approach to 3D STPP. While previous work provides a foundation, its direct extension overly restricts the intensity function and leads to computational challenges. In response, we introduce a decomposable parametrization for the integral network using ProdNet. This approach, leveraging the product of simplified univariate graphs, effectively sidesteps the computational complexities inherent in multivariate computational graphs. We prove the consistency of AutoSTPP and validate it on synthetic data and benchmark real-world datasets. AutoSTPP shows a significant advantage in recovering complex intensity functions from irregular spatiotemporal events, particularly when the intensity is sharply localized. Our code is open-source at https://github.com/Rose-STL-Lab/AutoSTPP.

==> secs/back.tex <==

% \paragraph{Temporal Point Processes.}
% A temporal point process (TPP) is a counting process $N(t)$, representing the number of events that occurs before time $t$. It is characterized by a scalar non-negative intensity function $\lambda^*(t)$. Given the history events before time $t$, $\mathcal H_t := \{t_1, ..., t_n\}_{t_n \leq t}$, the intensity function quantifies the event arrival rate at $t$, and is formally defined as 
% $$
% \lambda^*(t):=  \lim_{\Delta t \to 0}\frac{\mathbb{E}[ N(t, t+ d t)|\mathcal H_{t}]}{ dt}.
% $$
% The notation $*$ is from \cite{daley2007introduction} to indicate the intensity is conditional on the past but not including the present. One  example of TPP is  Hawkes process \citep{hawkes1971spectra}, characterized by
% \begin{align}
%     \lambda^*(t) = \mu + \alpha \sum_{t_i < t} \exp(-\beta(t-t_i)), \label{eqn:hawkes}
% \end{align} 
% where $\mu, \alpha, \beta$ are scalars. The arrival of a new event results in a sudden increase of intensity, and the influence of this event will decay exponentially. $\mu$ is the base intensity representing the rate of an event happening on its own.

\paragraph{Spatiotemporal Point Process.} \label{sec:spatialtemporal-point-process}
%
The spatiotemporal point process (STPP) models the number of events $N( \T{S} \times (a,b) )$ that occurred  in  the Cartesian product of the spatial domain $\mathcal{S} \subseteq \mathbb R^d$ ($d$ is the spatial dimensionality) and  the time interval $(a, b]$. It is characterized by a non-negative  \textit{space-time intensity function}  given the history $\mathcal{H}_t:= \{(\V{s}_1, t_1), \dots, (\V{s}_n, t_n)\}_{t_n \leq t} $: 
\begin{equation}
\lambda^*(\mathbf s,t) := \lim_{\Delta \mathbf{s}  \to 0, \Delta t  \to 0} \frac{\mathbb{E} [ N(B(\V{s},\Delta \V{s})  \times  (t, t+\Delta t)) | \mathcal H_t]}{ B(\mathbf s, \Delta \mathbf s) \Delta t  }
\label{eqn:def_stpp}
\end{equation}
 which is the probability of finding an event in an infinitesimal time interval $(t, t+ \Delta t ] $ and an infinitesimal spatial ball $\T{S}= B(\mathbf s, \Delta \mathbf s)$ centered at location $\V{s}$. Alternatively, an STPP can be seen as a TPP with a conditional spatial distribution $f^*(\mathbf s|t)$, such that $\lambda^*(\mathbf s, t) = \lambda^*(t) f^*(\mathbf s |t) $.
 
% \paragraph{Spatiotemporal Point Processes}

% Spatiotemporal point process (STPP) extends Temporal Point Process to the spatial domain. It models the number of events $N(\mathbf{s}, t)$ that occurred during the interval $(0, t]$ in the spatial domain $S \subseteq \mathbb{R}^2$ . The conditional intensity function is
% \begin{align*}
%     \lambda^{*}(\mathbf{s}, t):=\lim _{\Delta t \rightarrow 0, \Delta \mathbf{s} \rightarrow 0,} \frac{\mathbb{E}\left[\Delta N(\mathbf{s}, t) \mid \mathcal{H}_{t}\right]}{\Delta t \Delta \mathbf{s}}
% \end{align*}
% which models the number of events in an infinitesimal time interval $[t, t+\delta t]$ and an infinitesimal spatial ball $B(\mathbf{s}, \Delta \mathbf{s}) .$ Similarly, $\mathcal{H}_{t}:=\left\{\left(\mathbf{s}_{1}, t_{1}\right),\left(\mathbf{s}_{2}, t_{1}\right), \ldots,\left(\mathbf{s}_{n}, t_{n}\right)\right\}$ represents all spatiotemporal events up to time $t$.

\paragraph{Neural Point Processes.}
Neural  Point Process~(NPP) models  combine DNNs with point processes to increase their capacity. State-of-the-art NPPs first encode the events into hidden states. For temporal NPP, if the inter-event function is as simple as a scalar kernel function \citep{du2016recurrent}, then the integral is easy, but the model is less expressive. On the other hand, if the inter-event function is high dimensional  \citep{mei2016neural, zuo2020transformer}, then the model gains stronger expressive power at the cost of requiring numerical integration. For spatiotemporal NPP \citep{chen2020neural, zhou2022neural}, they use a non-negative activation function to map the hidden states to a scalar, i.e., the temporal intensity immediately after an event, and a conditional spatial distribution. The change of intensity between events is represented using a decay function or a Neural-ODE. The conditional spatial distribution is represented by a kernel mixture or a normalizing flow. Nevertheless, all models assume a continuous transformation of the intensity function and have limited expressivity. 

% By parametrizing the intensity function as $\lambda^*_{\theta}(t)$, the log likelihood of an event sequence $\{t_1, ..., t_N\}$  observed in time interval $[0, T]$ is 
% $$
% \mathcal L(\theta|\{t_1, ..., t_N\})= \sum_{i=1}^N \log \lambda^*(\V{s}_i,t_i^-) -\int_{ \mathcal{S}} \int_0^t \lambda^*(\V{u},\tau) d\V{u}d\tau.
% $$
% As the intensity is discontinuous at every event arrival $t_{i}$, $t_{i}^{-}$ denotes the intensity immediately before the $i$-th event. The second term is usually  evaluated separately for each inter-event interval $(t_i, t_{i+1})$. 

%  We found in our experiments that the numerical integration errors may prevent the model from recovering the true underlying intensity, see Figure \ref{fig:numint}. 



==> secs/backup.tex <==


\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/shakyHawkesRNN.pdf}
        \label{fig:mean and std of net14}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}  
        \centering 
        \includegraphics[width=\textwidth]{figs/shakyHawkesINT.pdf}
        \label{fig:mean and std of net24}
    \end{subfigure}
    \vspace{-7mm}
    \caption[ The average and standard deviation of critical parameters ]
    {\small Visualizations of the true conditional intensity $\lambda^*(t)$ and the learned conditional intensity on the \textit{Shaky Hawkes} dataset. Left: comparison of intensities learned with state-of-the-art  models. Right: comparison of intensities learned with different integration methods.} 
    \label{fig:mean and std of nets}
\end{figure*}



\begin{table*}[ht!]
\centering
\begin{adjustbox}{max width=\textwidth,center}
\centering
\begin{tabular}{c cc cc cc c}
\toprule
Model & \multicolumn{2}{c}{shakyHawkes} & \multicolumn{2}{c}{shiftHawkes} & \multicolumn{2}{c}{decayPeak} & earthquakesJP  \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}  \cmidrule(lr){8-8}
& MAPE & LL & MAPE & LL & MAPE & LL & LL\\ \midrule
CT-GRU \cite{mozer2017discrete}            & 0.2243 & -35.6063 & 0.1262 & -39.7173 & 0.1103 & -42.1959 & 5.9148 \\ 
Neural Hawkes \cite{mei2016neural}     & 0.2168 & -35.4043 & 0.1473 & -40.0411 & 0.1468 & -42.5548 & 7.0620 \\ 
RMTPP  \cite{du2016recurrent}            & 0.2562 & -35.6549 & 0.2630 & -39.7893 & 0.2183 & -42.7965 & 7.7663 \\
Transformer Hawkes \cite{zuo2020transformer} & 0.2812 & -36.1831 & 0.2316 & -40.6717 & 0.2342 & -43.3308 & 6.0588 \\ 
\midrule
\ours{} & \textbf{0.1843} & \textbf{-35.3762} & \textbf{0.0356} & \textbf{-39.3599} & \textbf{0.0226} & \textbf{-41.9678} & \textbf{8.6187} \\ 
\ours{} (w/ RNN) & 0.3353 & -37.9182 & 0.4675 & -44.0076 & 0.1107 & -42.3124 & 7.7730 \\ 
\bottomrule
\end{tabular} 
\label{tb:compare-baseline}
\end{adjustbox}
\caption{Comparison between our proposed model \ours{} (with or without RNN) and the state-of-the-art NPP models on three synthetic datasets and a real-world \textit{Earthquake Japan} dataset. Performance w.r.t.  Mean Absolute Percentange Error (MAPE) of the estimated conditional intensity $\lambda^*(t)$ and  Test log likelihood~(LL). } 
\end{table*}


\begin{table*}[ht!]
\centering
\begin{adjustbox}{max width=\textwidth,center}
\centering
\begin{tabular}{c cc cc cc c}
\toprule
Model & \multicolumn{2}{c}{shakyHawkes} & \multicolumn{2}{c}{shiftHawkes} & \multicolumn{2}{c}{decayPeak} & earthquakesJP  \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}  \cmidrule(lr){8-8}
& MAPE & LL & MAPE & LL & MAPE & LL & LL\\ \midrule 
Clenshaw-Curtis & 0.2197 & -35.5183 & 0.0541 & -39.4831 & 0.0312 & -41.9839 & 8.4299 \\ 
Monte Carlo & 0.1935 & -35.6090 & 0.0462 & \textbf{-39.3527} & 0.0378 & -41.9868 & 8.1906 \\ 
Taylor Expansion \citep{liu2020automatic} & 0.2004 & -35.3771 & 0.0999 & -39.7062 & \textbf{0.0224} & -41.9691 & 7.7142 \\ 
\midrule
\ours{} & \textbf{0.1843} & \textbf{-35.3762} & \textbf{0.0356} & -39.3599 & 0.0226 & \textbf{-41.9678} & \textbf{8.6187} \\
\bottomrule
\end{tabular} 
\label{tb:compare-numint}
\end{adjustbox}
\caption{Comparison between different integration methods using the same model on three synthetic dataset and a real-world \textit{Earthquake Japan} dataset. Performance w.r.t.  Mean Absolute Percentange Error (MAPE) of the estimated conditional intensity $\lambda^*(t)$ and  Test log likelihood~(LL). } 
\end{table*}





We evaluate \ours{} for learning temporal dynamics using both synthetic and real-world data. 

\subsection{Experimental Setup}
\textbf{Synthetic Datasets.}
Existing temporal point process models fail to capture the dynamics of the point process governed by multimodal or non-smooth current influence function. Here, we proposed and simulated three challenging synthetic datasets using Ogata's thinning algorithm \citep{chen2016thinning}. 
\begin{itemize}
    \item \textit{Shaky Hawkes process}: as illustrated by Figure \ref{fig:failedll}, it multiplies the influence function of the Hawkes process (see Equation \ref{eqn:hawkes}) by a cyclic function, such that the intensity becomes multimodal in long inter-event intervals.
    \item \textit{Delayed Peak process}: it features a uni-modal but non-smooth influence function. Each event's influence is initially 0; then it first increases and then decreases, following a bell-shaped curve.
    \item \textit{Shift Hawkes process}: as mentioned in Section \ref{sec:intro}, it describes the scenario in which a post becomes viral several hours after it is visible, such that there is a jump in the intensity between events. 
\end{itemize}
The detailed information of the synthetic datasets are deferred to the Appendix Section \ref{app:synthetic}.

\textbf{Real-world Datasets.} We use a real-world dataset, \textit{Earthquake Japan}, that includes the times and locations of all earthquakes in Japan from 1990 to 2020 with magnitudes of at least 2.5. It is gathered by \citet{chen2020neural}. 

\textbf{Evaluation Metrics.}
As shown by Figure \ref{fig:failedll}, a TPP model may yield a likelihood similar to the ground truth but fail to capture the correct intensity. Therefore, in addition to the likelihood~(LL), we show the Mean Absolute Percentage Error~(MAPE) of the estimated conditional intensity.

\textbf{Baselines.} We have two groups of baselines: 
\begin{itemize}
    \item \textit{Integration methods}: the baselines learn the point process using the same model as described by Equation \ref{eqn:same_influence} but with four different integration techniques: Taylor integration \citep{liu2020automatic}, the Clenshaw–Curtis quadrature, the Monte Carlo integration, and AutoInt. 
    \item \textit{Delayed Peak process}: it features a uni-modal but non-smooth influence function. Each event's influence is initially 0; then it first increases and then decreases, following a bell-shaped curve.
    \item \textit{Shift Hawkes process}: as mentioned in Section \ref{sec:intro}, it describes the scenario in which a post becomes viral several hours after it is visible, such that there is a jump in the intensity between events. 
\end{itemize}

%the first group follows the  model in \ref{eqn:same_influence}  but applies different numerical integration techniques. This group of baselines include \cite{liu2020automatic}'s Taylor approximation method \ref{app:taylor}, the Clenshaw–Curtis quadrature method \ref{app:cheby} and the Monte Carlo integration method. The first two methods approximate the neural network with orthogonal polynomials (Taylor and Chebyshev polynomials) and then rely on the easy integrability of polynomials. The third one is the most commonly used method for modeling the temporal point process.

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\includegraphics[width=\linewidth, trim={2mm 2mm 5mm 5mm},clip]{figs/traintime.png}
\end{center}
\vspace{-2mm}
\caption{Training speed comparison for different NPPs and numerical integration methods in seconds. The proposed \ours{} is fast. RMTPP is the fastest but suffers from poor prediction performance.}
\label{fig:speed_up}
\end{figure}

%In the second group, we include state-of-the-art NPP models, including RMTPP \citep{du2016recurrent}, Neural-Hawkes \citep{mei2016neural} and Transformer Hawkes \citep{zuo2020transformer}. Additionally, \cite{mozer2017discrete} proposed a continuous-time GRU that interpolates hidden states between events. It has a similar idea as Neural-Hawkes's continuous-time LSTM. So given that Neural-Hawkes is the only baseline that interpolates hidden states, we additionally include a CT-GRU variant of Neural-Hawkes to increase the diversity of our baselines. 

%RMTPP was proposed quite early; its current influence function is an exponential decay function and the decay rate is a scalar parameter across all sequences. For a fair comparison, we added a revised version of RMTPP that has its decay rate being also dependent on the hidden states. We also keep the original RMTPP and call it RMTPP original. Most baseline methods originally use a linear mapping from the hidden state to the intensity function. Given that our inter-event dynamic is complicated, we added ``deep mapping" variants of CT-GRU, CT-LSTM Neural-Hawkes, and Transformer Hawkes, which has a three-layer MLP mapping from the hidden states to the intensity function. By adding all these variants, we believe we have a fair coverage of possible TPP baselines.


In the second group, we include state-of-the-art methods with outstanding performance, including RMTPP \citep{du2016recurrent}, neural-Hawkes \citep{mei2016neural} and Transformer Hawkes \citep{zuo2020transformer}.



\subsection{Experimental Results}

Figure \ref{fig:speed_up}  visualize the run-time comparison of different methods. We can see that 


Table \ref{tb:prediction} compares the prediction  Mean Absolute Percentage Error (MAPE) and test log-likelihood for different methods on four datasets. We can see that 

\iffalse
\begin{table*}[ht!]
\centering
\begin{adjustbox}{max width=\textwidth,center}
\centering
\begin{tabular}{c cc cc cc c}
    \toprule
    Model & \multicolumn{2}{c}{shakyHawkes} & \multicolumn{2}{c}{shiftHawkes} & \multicolumn{2}{c}{decayPeak} & earthquakesJP  \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}  \cmidrule(lr){8-8}
     & MAPE & LL & MAPE & LL & MAPE & LL & LL\\ \midrule 
        AutoInt-GRU TPP & 0.6435 & -64.7072 & 0.4522 & -58.4046 & 0.4100 & -65.0632 & -2.6385 \\ 
        Chebyshev TPP SI & 0.2197 & -35.5183 & 0.0541 & -39.4831 & 0.0312 & -41.9839 & 8.4299 \\ 
        CT-GRU Hawkes Deep & 0.2432 & -36.3658 & 0.1235 & -39.6273 & 0.0708 & -42.1338 & 8.6817 \\ 
        CT-GRU Hawkes Linear & 0.2243 & -35.6063 & 0.1262 & -39.7173 & 0.1103 & -42.1959 & 5.9148 \\ 
        CT-LSTM Hawkes Deep & 0.1938 & -35.2895 & 0.1381 & -39.8087 & 0.1623 & -42.6656 & 9.7533 \\ 
        CT-LSTM Hawkes Linear & 0.2168 & -35.4043 & 0.1473 & -40.0411 & 0.1468 & -42.5548 & 7.0620 \\ 
        Monte Carlo TPP SI & 0.1935 & -35.6090 & 0.0462 & -39.3527 & 0.0378 & -41.9868 & 8.1906 \\ 
        RMTPP & 0.2216 & -35.4175 & 0.1515 & -39.8077 & 0.1660 & -42.5876 & 4.8615 \\ 
        RMTPP Original & 0.2562 & -35.6549 & 0.2630 & -39.7893 & 0.2183 & -42.7965 & 7.7663 \\ 
        Taylor TPP SI & 0.2004 & -35.3771 & 0.0999 & -39.7062 & 0.0224 & -41.9691 & 7.7142 \\ 
        Transformer Hawkes Deep & 0.2639 & -36.3195 & 0.2105 & -40.2917 & 0.1864 & -42.9732 & 3.8893 \\ 
        Transformer Hawkes Linear & 0.2812 & -36.1831 & 0.2316 & -40.6717 & 0.2342 & -43.3308 & 6.0588 \\ 
                \midrule
Ours & 0.1843 & -35.3762 & 0.0356 & -39.3599 & 0.0226 & -41.9678 & 8.6187 \\ Ours (w/ RNN) & 0.3353 & -37.9182 & 0.4675 & -44.0076 & 0.1107 & -42.3124 & 7.7730 \\ 
\bottomrule
\end{tabular} 
\label{tb:prediction}
\end{adjustbox}
\caption{Test log likelihood~(LL) on synthetic and real-world data. Mean absolute percentage error~(MAPE) of the estimated conditional intensity $\lambda^*(t)$ on synthetic data. Comparison between ours model (with or without deep sequence model) and the baseline models.} 
\end{table*}
\fi


